Towards A Unified Neural Architecture for Visual Recognition and Reasoning

Recognition and reasoning are two pillars of visual understanding. However, these tasks have an imbalance in focus; whereas recent advances in neural networks have shown strong empirical performance in visual recognition, there has been comparably much less success in solving visual reasoning. Intuitively, unifying these two tasks under a singular framework is desirable, as they are mutually dependent and beneficial. Motivated by the recent success of multi-task transformers for visual recognition and language understanding, we propose a unified neural architecture for visual recognition and reasoning with a generic interface (e.g., tokens) for both. Our framework enables the principled investigation of how different visual recognition tasks, datasets, and inductive biases can help enable spatiotemporal reasoning capabilities. Noticeably, we find that object detection, which requires spatial localization of individual objects, is the most beneficial recognition task for reasoning. We further demonstrate via probing that implicit object-centric representations emerge automatically inside our framework. Intriguingly, we discover that certain architectural choices such as the backbone model of the visual encoder have a significant impact on visual reasoning, but little on object detection. Given the results of our experiments, we believe that visual reasoning should be considered as a first-class citizen alongside visual recognition, as they are strongly correlated but benefit from potentially different design choices.

==> content/experiments_backup.tex <==
\section{Experiments}

%\chen{TODO(chen): When discuss probing, may mention that even better binding may emerge with large-scale pre-training. We may also have a limitation paragraph in conclusions.}

We showcase our model on two spatiotemporal reasoning tasks, CATER~\citep{girdhar2019cater} and ACRE~\citep{zhang2021acre}, and perform ablations over them.  The encoder and decoder of the model is also initialized from a pre-trained ImageNet classification checkpoint, on top of which all visual and reasoning tasks are further optimized on.
%In these experiments we apply only one switch between tasks, optimizing object-detection first before learning to do reasoning.  Despite our proposed approach being more general, we are still able to demonstrate a variety of interesting results under this setting. 
All reported experiments were performed on 32 Dragonfish TPUs per run.

% \subsection{Overview of Datasets and Object Detection Pretraining}
% % Describe our pretraining procedure.
% The visual environments of both CATER and ACRE are composed of CLEVR objects.

\subsection{CATER}
We first evaluate our model on the CATER task.  CATER is composed of videos of CLEVR~\citep{johnson2017clevr} objects moving and, importantly, occluding each other.  Conceptually, it is meant to simulate the shell game, where the objective is to locate the final position of a ball that is hidden under a cup and shuffled with other cups.  In the CATER task, larger objects can occlude smaller objects visually, with respect to the camera viewpoint.  Furthermore, objects can also completely cover up smaller objects and move around with them, effectively moving multiple objects at once while occluding them entirely from view.  As in the shell game, the CATER task is to locate the final position of a unique golden object, named the ``snitch", where locations are represented as units on a 6x6 grid.  Therefore, the problem can be interpreted as a 36-way classification problem. Whereas the CATER dataset features an additional split where the camera viewpoint can also move freely over the course of the video, we focus on the static camera setting in our experiments.  A visual demonstration of a sample CATER task is provided in Figure \ref{fig:cater}.

\begin{figure}
  \centering
  \includegraphics[width=0.99\linewidth]{content/figures/cater_frames.png}
  \caption{Example frames from a CATER video. %  Frame 0 shows the initialization of the video.  Frame 20 shows objects being picked up and moved around.  Larger cones can cover up smaller objects; in Frame 70, the large green cone completely covers the cyan cone.  As the green cone moves, shown in Frame 100, it also moves any objects it covers, such as the cyan cone.  Interpreting the ground as a consistent but invisible 6 by 6 grid, 
  The task is to determine the final location of the golden snitch, which may be occluded or covered throughout the video, as one of 36 locations.}
  \label{fig:cater}
\end{figure}

By default, each CATER video contains 301 frames.  We follow the experimental setup in ALOE~\citep{ding2021attention} to generate each training example; uniformly random sampling is utilized to select 80 frames from the full video, which are then reordered to preserve temporal order, and each frame is resized to 64x64 resolution.  We also perform evaluation on 80 frame subsequences, but space their indices as evenly as possible.  We utilize a batch size of 256, and find convergence in 7,000 steps.  We find that using 3500 warmup steps, a learning rate of $3e^{-4}$ with a linear scheduler, and the Adam optimizer~\citep{kingma2014adam} with weight decay factor 0.05, generally produces the best results.  For other hyperparameter settings, we either match the configurations used by ALOE, or select them from validation set performance.  When adapting our framework on CATER, we concatenate only the first token from the encoder output of each frame and expose it to the decoder; we also provide ablations over the number of tokens to use per frame in Table \ref{cater_ablations}. 
%\chen{Do we have a list of the other hyper parameters and what are their values}

As a default baseline, we first attempt to train our proposed framework to solve the CATER task directly.  In this baseline, no recognition task information is provided anywhere to the framework; it is tasked with trying to solve the reasoning task directly from the provided dataset with random weight initialization.  We refer to this baseline approach as “Ground-Up”.  In Table~\ref{cater_ablations}, we discover that it struggles to perform reasoning; our model achieves 18.10\% test accuracy when using a ResNet Transformer encoder backbone, and a mere 4.36\% when using a pure Vision Transformer encoding backbone.  For reference, a random guess on the location would be accurate 2.78\% of the time. %\chen{(1) Need to explain how we set the hparams of both ResNet-C and ViT-B baselines.}% (2) Let's discuss if we should treat ALOE as a ``baseline''. If so, need to discuss why ALOE can be trained from scratch.}

We then evaluate our multi-task model formulation, by training on the object-detection task before learning how to perform reasoning.  Firstly, however, to even train on object detection we require ground truth bounding box supervision.  As these labels are not present in the CATER dataset, we use the annotations from the LA-CATER dataset~\citep{shamsian2020learning}.  The LA-CATER dataset is generated to be identical to the CATER domain; it features the same camera configuration, the same usage of CLEVR objects, and the same number of possible objects per scene.  Utilizing LA-CATER therefore enables us to first train our framework on the recognition task of object-detection in a visually consistent setting, before proceeding to learn the desired reasoning task.  We discover that our end-to-end model trained in this way is able to perform the CATER task with 74.09\% test accuracy using a ResNet Transformer encoder and 56.64\% using a Vision Transformer backbone.  Our end-to-end multitask model is therefore able to outperform the default ALOE model, which achieves 70.6\% test accuracy.  Its performance is also comparable with the ALOE model that uses a task-specific L1 loss, which achieves $74.0 \pm 0.3\%$ (See Appendix) %(Table~\ref{cater_benchmark})
.  In contrast, we do not use any extra auxiliary task-specific losses in our setup.  We therefore conclude that the addition of the general object-detection task helps the model perform spatio-temporal reasoning in an end-to-end unified model.
%\boqing{At least two factors might have contributed to the superior results: the detection task and additional data in LA-CATER, so perhaps re-phrase this sentence?}.
Given ALOE's finding that object-centric abstractions of the input are important for reasoning, which they leverage a pre-trained MONET model to generate, we take this as a preliminary sign that the model forms strong object-centric representations implicitly. %\chen{This section would be more focused if we skip the ViT results since they are discussed later in a separate paragraph.}

We also explore whether object-detection as an objective is generally useful, or if the benefits are only limited to the visual domain of the reasoning task.  In other words, we investigate if there are inherent properties of object detection that could potentially enable the learning of object-centric abstractions that can extend beyond visual domains, and still be useful in enabling reasoning capabilities.  We test this in our model by evaluating CATER performance with object-detection pre-training on the MS-COCO dataset.  Composed of natural images, the MS-COCO dataset is visually dissimilar from the synthetic CATER environment, and the two datasets share no overlapping object classes.  However, we find that our method still achieves 69.79\% on test performance using a ResNet Transformer encoder.  Therefore, even though it is trained for object detection on a completely different visual domain, we see that our method is still able to exhibit reasoning capabilities, even beating the default ALOE performance.  Whereas ALOE requires pretraining a separate model on the same visual demonstrations from the same domain in a pipeline-style approach, we demonstrate that our model is still able to perform reasoning in an end-to-end way, leveraging object-detection capabilities on out-of-domain data.  This is a surprising and powerful result that further diminishes the need for task-specific considerations or pipeline-style approaches, and hints at the efficacy of object detection as a general task. 
%\boqing{Summarize the results here and those in the last paragraph into a table, and make the caption as self-contained as possible?}

Furthermore, we ablate over the number of tokens provided by the encoder to the decoder, and find that using only one token per frame works the best.  This is potentially due to the singular token containing enough information to solve the task of locating the snitch.  To provide intuition on this, we visualize if the token contains an accurate belief over the location of the snitch at arbitrary frames in our probing experiments below.

\begin{table}[t]
\caption{Ablations on the CATER benchmark.  We demonstrate that choices between encoder architectures (between using intermediate features from a ResNet as patch embeddings versus linear projections of patches as in a ViT) are considerable; using a ResNet + Transformer encoder backbone consistently achieves better reasoning performance.  We also ablate over the recognition task and between not using one, training on LA-CATER object detection, as well as MS-COCO object detection.  We also demonstrate that for the CATER task, performance does not improve when using more than 1 bottleneck token.  This is encouraging, as it shows that the information for solving a complex spatiotemporal reasoning task can be condensed into a small number of tokens. } %TODO: Explain this portion. the encoder backbone choice show that the ResNet + Transformer achieves better performance than the Vision Transformer.  Furthermore, we demonstrate that one slot performs better than multiple slots, in the CATER environment.
\label{cater_ablations}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llll}
\multicolumn{1}{c}{\bf Encoder Backbone}  &\multicolumn{1}{c}{\bf Recognition Task}   &\multicolumn{1}{c}{\bf Tokens per frame}    &\multicolumn{1}{c}{\bf CATER Top 1 (Static)}
\\ \hline \\
ResNet + Transformer & None (Ground-Up)& 1 (slot)     & 18.10\%\\
Vision Transformer & None (Ground-Up)& 1 (slot)     & 4.36\%\\
ResNet + Transformer & LA-CATER ObjDet   & 1 (slot) & \textbf{74.09\%}\\
Vision Transformer & LA-CATER ObjDet   & 1 (slot)  & 56.64\%\\
ResNet + Transformer & LA-CATER ObjDet   & 10 (slots) & 71.68\%\\
%Vision Transformer & LA-CATER ObjDet   & 10 (slot)  & \text{TODO}\%\\
ResNet + Transformer & MS-COCO ObjDet & 1 (slot) & 69.79\%\\
\end{tabular}%
}
\end{table}
% \chen{There are many different factors we change in this table. Explain what they are in the caption.}

% \begin{table}[t]
% \caption{
% % Comparison to supervised pretraining.
% \textbf{
% End-to-end visual pretraining vs. supervised pretraining.}
% We compare our proposed pretraining with traditional classification or detection pretraining.
% IV-CL significantly outperforms existing supervised alternatives.
% }
% % \vspace{-1em}
% \vspace{-3mm}
% \label{supervised_pretrain}
% \begin{center}
% \begin{tabular}{cccc}
% \toprule
% Encoder Backbone & Recognition Task & Tokens per frame & CATER Top 1 (Static)\\
% \midrule
% ResNet + Transformer & None (Ground-Up)& 1 (slot)     & 18.10\%\\
% Vision Transformer & None (Ground-Up)& 1 (slot)     & 4.36\%\\
% ResNet + Transformer & LA-CATER ObjDet   & 1 (slot) & \textbf{74.09\%}\\
% Vision Transformer & LA-CATER ObjDet   & 1 (slot)  & 56.64\%\\
% ResNet + Transformer & LA-CATER ObjDet   & 10 (slots) & 71.68\%\\
% %Vision Transformer & LA-CATER ObjDet   & 10 (slot)  & \text{TODO}\%\\
% ResNet + Transformer & MS-COCO ObjDet & 1 (slot) & 69.79\%\\
% \midrule
% IV-CL & CATER & \textbf{70.03\%} & \textbf{93.03\%} \\
% \bottomrule
% \end{tabular}
% \end{center}
% % \vspace{-1em}
% \vspace{-5mm}
% \end{table}

Lastly, we note that in all of our experiments, the ResNet Transformer encoder backbone is much more performant than the Vision Transformer encoder backbone.  The performance disparity when applied to a reasoning task is a surprising result, since both architectures achieved similarly high AP50 performance on LA-CATER (81.53 for the ResNet Transformer, and 82.44 for the Vision Transformer).  We therefore believe that convolutional inductive bias is still important.  In particular, as ALOE has demonstrated the importance of object-centric abstractions of input, perhaps the convolutional structure is more adept at isolating and encoding object-centric information than the linear operation employed by the vanilla Vision Transformer encoding scheme.  We believe this is a signal that architectural considerations will be important when designing solutions to reasoning problems, and that simply reusing settings that work on pure visual recognition tasks can potentially inhibit performance. %\chen{Another possible explanation might be ViT needs more pretraining (as we show in the other work).}
\begin{figure}
  \centering
  \includegraphics[width=0.99\linewidth]{content/figures/acre_frames.png}
  \caption{An example of the ACRE task.  The first three images represent context panels, which expose the state of the underlying platform to the model.  The model must predict the platform state for the two query configurations, shown as Query 1 and Query 2.  The result of Query 1 is undetermined; although we know the purple cylinder does not light up the platform, we do not have enough information regarding the blue metal cube, as the signal in Context 2 may or may not be the result of the other objects present.  That Query 2 would not light up the platform can be deduced from Contexts 1 and 3.  For ACRE, six context images are provided, with four associated queries.}
  \label{fig:acre}
\end{figure}

\subsection{ACRE} \label{sec:acre}
%\chen{Where are the tables we compare with prior SoTA?}
We also evaluate our model on the ACRE task, which tests causal inference capabilities.  ACRE is based off the Blicket experiment from developmental psychology~\citep{gopnik2000detecting}.  In the original formulation, a machine lights up when certain objects, called ``Blickets" are placed on it.  Preschool-aged children are tasked with determining which objects are Blickets, given demonstrations of certain object configurations and their resulting effects on the machine.  In the ACRE task, CLEVR objects are placed on a fixed platform, which glows or remains dim depending on the ``Blicketness" properties of the objects.  The model is provided with six context frames demonstrating different combinations of objects and their corresponding platform state, as well as a query frame containing an object combination that the model is expected to predict the result of.

There are four types of reasoning tasks the model is tested on, categorized by question types: direct, indirect, screened-off, and backward-blocking.  The potential answers for each of these questions is either that the platform's state is on, off, or unable to be determined.  In a direct question, the query combination is previously observed during one of the provided context trials; the model must be able to recognize it from the context and reference it to retrieve the answer.  In an indirect question, the query combination is novel, and the result must be deduced from several frames.  In screen-off questions, the model must learn the dynamic that as long as one Blicket object is present, the entire combination would turn the machine on.  Lastly, in the backward-blocking questions, the model must correctly deduce that the query combination cannot be ascertained from the available contexts.

% \begin{table}[t]
% \caption{Ablations over the number of tokens used per frame reveal the benefit of using bottleneck tokens.  Furthermore, despite achieving a high AP50 on LA-CATER, the Vision Transformer underperforms compared to the ResNet + Transformer when the same bottleneck is applied.}
% \label{acre_ablations}
% \begin{center}
% \begin{tabular}{llll}
% \multicolumn{1}{c}{\bf Encoder Backbone}  &\multicolumn{1}{c}{\bf Tokens per frame}   &\multicolumn{1}{c}{\bf ACRE (Comp Split)} &\multicolumn{1}{c}{\bf ACRE (LA-CATER AP50)}
% \\ \hline \\
% %ResNet + Transformer  & 400 (patches) & 39.30\%   & 88.70\%\\
% Vision Transformer  & 10 (slots)  & 53.61\%   & 91.91\% \\
% ResNet + Transformer  & 10 (slots)  & 59.35\%   & 88.50\%\\
% ResNet + Transformer  & 20 (slots)  & \textbf{60.93\%}   & 92.35\%\\
% ResNet + Transformer  & 1 (slot)   & 46.28\%   & 87.28\%\\
% \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[t]
% \caption{Ablations over encoder backbone choice, recognition task, and number of slot tokens on the ACRE environment.} %TODO: Explain this portion. the encoder backbone choice show that the ResNet + Transformer achieves better performance than the Vision Transformer.  Furthermore, we demonstrate that one slot performs better than multiple slots, in the CATER environment.
% \label{acre_ablations}
% \begin{center}
% \begin{tabular}{llll}
% \multicolumn{1}{c}{\bf Encoder Backbone}  &\multicolumn{1}{c}{\bf Recognition Task}   &\multicolumn{1}{c}{\bf Tokens per frame}    &\multicolumn{1}{c}{\bf ACRE (Comp)}
% \\ \hline \\
% %ResNet + Transformer & LA-CATER ObjDet   & 1 (slot) & \textbf{74.09\%}\\
% %Vision Transformer & LA-CATER ObjDet   & 1 (slot)  & \text{TODO}\%\\
% ResNet + Transformer & LA-CATER ObjDet   & 10 (slots) & 81.65\%\\
% Vision Transformer & LA-CATER ObjDet   & 10 (slots)  & 78.79\%\\
% %ResNet + Transformer & MS-COCO ObjDet & 1 (slot) & \text{TODO}\%\\
% ResNet + Transformer & MS-COCO ObjDet & 10 (slot) & \textbf{83.81}\%\\
% \end{tabular}
% \end{center}
% \end{table}

\begin{table}[t]
\caption{Comparisons across visual perception objectives and datasets.  We choose the objectives of Object Detection and Visible Object Detection to determine if recognition tasks that require strong spatial localization ability indeed help reasoning performance under our framework.  We contrast this property with other visual perception objectives such as Count All Objects and Count Unique Objects in a scene; such perception objectives do need to understand the visual scene to some degree but do not explicitly require spatial localization to understand where in the picture each object is.  We also find a balance in the Snitch Detection task, which requires moderate spatial localization.  We generally find that utilizing visual recognition tasks that require understanding spatial localization result in the best reasoning performance.}
\label{objective_ablations}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llll}
\multicolumn{1}{c}{\bf Dataset} &\multicolumn{1}{c}{\bf Visual Recognition Task}  &\multicolumn{1}{c}{\bf ACRE (Comp)}   &\multicolumn{1}{c}{\bf CATER Top 1 (Static)}
\\ \hline \\
LA-CATER & Object Detection  & 67.27\%   & \textbf{74.09\%}\\
LA-CATER & Visible Object Detection  & 81.65\%   & 73.44\% \\
LA-CATER & Count All Objects  & 44.04\%   & 68.36\%\\
LA-CATER & Count Unique Objects  & 41.48\%   & 64.78\%\\
LA-CATER & Snitch Detection  & 79.70\%   & 72.66\%\\
MS-COCO & Object Detection  & \textbf{83.81\%}   & 69.79\%\\
\end{tabular}%
}
\end{table}
% \chen{Briefly summarize what are the objectives and why we pick them.}

% \begin{table}[t]
% \caption{Comparisons across visual perception objectives and datasets.}
% \label{objective_ablations}
% \begin{center}
% \begin{tabular}{llll}
% \multicolumn{1}{c}{\bf Dataset} &\multicolumn{1}{c}{\bf Visual Recognition Task}  &\multicolumn{1}{c}{\bf ACRE (Comp)}   &\multicolumn{1}{c}{\bf CATER Top 1 (Static)}
% \\ \hline \\
% LA-CATER & Object Detection  & 67.27\%   & \textbf{74.09\%}\\
% LA-CATER & Visible Object Detection  & 81.65\%   & 73.44\% \\
% LA-CATER & Count All Objects  & 44.04\%   & 68.36\%\\
% LA-CATER & Count Unique Objects  & 41.48\%   & 64.78\%\\
% LA-CATER & Snitch Detection  & 79.70\%   & 72.66\%\\
% MS-COCO & Object Detection  & \textbf{83.81\%}   & 69.79\%\\
% %MS-COCO Instance Segmentation  & 45.74\%   & 70.57\%\\
% \end{tabular}
% \end{center}
% \end{table}

As in the CATER experiments, we utilize a model trained on the object detection task using the LA-CATER dataset.  We reuse many of the same hyperparameter configurations from the CATER setup, except with 3000 warmup steps and 50,000 total training steps.

% This mirrors the setup from ALOE, which found that a visual encoder trained to handle CATER-style visual inputs could be reused out of the box successfully for ACRE purposes.  %We also reuse many of the same hyperparameter configurations from the CATER setup.  

%\chen{We organize the first two subsections by datasets, which is fine. It becomes confusing where to find the relevant discussions for Table 2 since it covers both datasets. It would be cleaner to either (1) first describe both datasets, then organize the subsections by the key ablations (backbone, inductive bias, pretraining objective, pretraining dataset); or (2) compare with SoTA on CATER and ACRE in section 4.1 and 4.2 respectively, then add a new subsection to discuss the impact of perception objectives, since it's the main results of our paper. I prefer (1) but (2) might be easier to rewrite since it requires fewer changes.}

We first investigate how different types of visual recognition tasks can enable reasoning capabilities in Table~\ref{objective_ablations}.  We therefore ablate over a variety of different tasks.  In LA-CATER Object Detection, the visual recognition is tasked with predicting the bounding boxes and shapes of all objects in the scene, hidden or visible; for MS-COCO the model predicts the bounding boxes and class labels.  In Visible Object Detection, the model is only asked to predict the bounding boxes and shape labels for all visible objects from the camera perspective.  In Count All Objects and Count Unique Objects, the model is tasked with predicting the number of total objects in the scene, and the number of unique shapes in the scene, respectively; notably, these objectives do not require the model to learn strong spatial localization.  Lastly, the Snitch Detection objective encourages the model to predict the bounding box location of the golden snitch.  We find that the best performance on ACRE is achieved through visual objectives that involve spatial localization.  Indeed, the top two performances on both ACRE and CATER utilize the Object Detection task: on MS-COCO and visible objects from LA-CATER for ACRE, and LA-CATER and visible LA-CATER for CATER.  Learning to predict hidden or occluded objects, as in the complete LA-CATER Object Detection, may not be helpful for the ACRE task since there are no fully occluded objects in the environment. We also notice that the visual recognition tasks that do not require explicit spatial localization, such as Count All Objects or Count Unique Objects, perform worst on their respective reasoning environments.  Furthermore, we find that the snitch detection performs well; on CATER, this is to be expected since it is directly useful for the final reasoning objective.  Overall, these results support the hypothesis that perceptual tasks that learn spatial localization of objects are beneficial for unlocking reasoning capabilities.

% Bottlenecking experiments.
% We first investigate the inductive bias regarding the type of tokens that can be learned by the encoder and used by the decoder in Table~\ref{acre_ablations}.  By default, when we train our model using a ResNet+Transformer encoder backbone and utilize the entire 400 self-attention token output of the encoder for decoding, the LA-CATER pre-trained model achieves an AP50 of 88.70\% on the object-detection test set.  When we freeze the encoder, to preserve the learned features, and continue training the decoder on top to perform the ACRE task, it achieves a validation accuracy of 39.30\%.  On the other hand, when we use the ``slot'' tokens to condense visual information per frame, we see an increase in performance.  When we train our model with the same encoder backbone, but limited to ten slot tokens, it achieves an AP50 of 88.50\% for object detection and 59.35\% for ACRE performance.  What this demonstrates is that although the inductive bias of token type does not affect object detection performance greatly, it has severe impact on reasoning capability. % Explain why this might be the case. 
%The cross-attention token may explain this increase in performance due to...
% The results are also consistent; when we modulate the bottleneck from 10 slot tokens to 1, we see a performance of 46.28\%, which still outperforms using all of the SA tokens.  Furthermore, when we increase the bottleneck to 20 slot tokens, we observe 92.35\% AP performance on object detection and 60.93\% on the ACRE task.

% Encoder-backbone experiments.
% Table~\ref{acre_ablations} also compares the differences between the ResNet+Transformer and the ViT encoder backbone, we observe the same trend as in CATER: Although the ViT encoder outperforms its ResNet counterpart in object detection, its reasoning performance is considerably lower.

%....%please expand on this, what are the main takeaways

\subsection{Probing}

%\chen{What does the color coding correspond to?}
\begin{figure}
  \centering
  \includegraphics[width=0.99\linewidth]{content/figures/cater_probing.png}
  \caption{Visualizing the object-centric information in a frozen, learned CATER embedding via probing.  We demonstrate the result of predicting the snitch location, as well as the locations of other objects in the scene.  We find that the frozen CATER embedding is adept at modeling the location of the snitch.}
  \label{fig:snitch}
\end{figure}

\begin{figure*}
  \centering
  \includegraphics[width=0.99\linewidth]{content/figures/test_probe_titled.png}
  \caption{We visualize the true positive bounding box and shape predictions for each of the ten bottleneck embeddings in a frozen ResNet + Transformer encoder using probing.  Note that each token seems to be adept at encoding one or a few objects well.}
  \label{fig:probes}
\end{figure*}

% \paragraph{Representation Probing.} We are interested in investigating the encoder's bottleneck embeddings to determine if they exhibit some object-centric or localized properties; as the decoder directly references them to solve tasks, their representational quality directly impacts performance.  One way to evaluate the information contained within the embeddings is through probing; after designating a set of embeddings of interest (or combinations thereof, in the general case), we can probe if they contain object-centric information such as bounding box coordinates or class labels.  The object detection training framework can be reused with two changes: we randomly sample embeddings from the investigation set at each training iteration to attempt the object detection task, and we freeze the encoder so that the representations are purely evaluated and are not modified or supervised further.  After our decoder is trained to perform probing in such a fashion, we can apply it during inference to evaluate every embedding of interest.
% Intuitively, if the encoder chooses to organize visual information in an object-centric fashion, it is expected that every probed embedding can successfully detect only one or few objects in an image, as information about other objects and their corresponding attributes are \textit{routed} to other embeddings. %It is also expected that when combined together, the objects successfully detected by all embeddings should be complete and cover every object in the scene.

% We note that since our framework also models probing as sequence prediction, it can be easily extended to incorporate arbitrary available ground-truth probing information available in a given domain, such as color and material, through constructing an appropriate target prediction sequence.  Overall, our unified framework naturally enables flexible probing functionality, thus allowing users to interpret and analyze the internal representations of the model with minimal adjustment.

% We perform probing experiments to understand the information encoded in the learned embeddings under our unified architecture.  Firstly, we investigate the singular bottleneck embedding learned by a CATER model that used the LA-CATER Object Detection visual recognition task with a ResNet + Transformer backbone.  Probing can be performed naturally under our proposed framework by first simply loading and freezing the encoder of a learned model, and then proceeding to learn an autoregressive decoder on the object detection task.  For example, to probe the CATER model, we can learn an autoregressive decoder to predict the location of the snitch, to verify if such information is encoded in the embedding.  We visualize our predictions in Figure \ref{fig:snitch}, and demonstrate that indeed the 

We perform probing under the setup described in the Methods section, to understand the information encoded in the learned embeddings under our unified architecture.  We begin by investigating the singular bottleneck embedding learned by a CATER model under our proposed framework that pretrained with an LA-CATER Object Detection task and utilized a ResNet + Transformer backbone.  We load and freeze the encoder of the learned CATER model, and proceed to train an autoregressive decoder on the snitch detection task, LA-CATER Visible Object Detection, and LA-CATER Object Detection.  We then visualize our predictions in Figure \ref{fig:snitch} for randomly selected frames, and demonstrate qualitatively that the learned embedding consistently encodes an accurate prediction of where the snitch is at any given time, regardless of the probing objective.  What this shows is that the frozen bottleneck always encodes the snitch location information, for which a learned probing autoregressive decoder can be cheaply trained to read out.  As tracking where the snitch is over multiple frames is indeed a necessity to solve the CATER task, and it is therefore a nice result that such information can be shown to be stored in the singular bottlenecking token.

%\chen{Explain why this matters, the frozen bottleneck always encodes the snitch location information, which can then be decoded by the prober.}

We also perform probing experiments on a ResNet Transformer encoder that was previously trained on LA-CATER for the object detection task using ten bottleneck embeddings to understand how the reasoning models for CATER and ACRE are initialized.  As we utilize this object detection pretraining procedure before each of the two reasoning tasks we evaluate on, the embedding outputs of this encoder are especially interesting to investigate in order to understand how they can potentially enable reasoning capabilities.  We freeze the encoder, and proceed to learn an autoregressive decoder on the LA-CATER object detection task, but selecting one token at random each iteration.  After convergence, we use the trained decoder to evaluate each individual bottleneck token of the encoder by qualitatively visualizing their predicted bounding boxes on a random LA-CATER test set frame.

In Figure \ref{fig:probes_annotated} we display all the predicted bounding boxes with a confidence score above 90\% for each token.  We notice three things - firstly, no token is encoding every object. 
%\chen{Why encouraging? Probably the three observations combined are encouraging, because it implies that object-centric tokens emerge via the OD objective and the token inductive bias.} %todo: maybe chen can explain this better - because it isnt a distributed representation.
In fact, there exists a token, token number 6, that does not appear to encode any object strongly.  This is not of particular issue, as there are ten total ``slot" tokens learned, but only eight objects in the scene.
Secondly, we discover that with the exception of number 6, the tokens are able to predict one or a few objects exceptionally accurately.  We visualize these clean predictions in Figure \ref{fig:probes}, and display their corresponding predicted shapes as well.  These results demonstrate that individual tokens are able to not only understanding where certain objects are but their properties as well.
Lastly, we observe that despite each token representing one or a few objects well, all of the objects in the scene are accounted for and there are few overlaps.  Therefore we discover %the surprising result 
that in combination, the tokens learned under our framework are able to collectively represent an entire scene in terms of its objects well, while encoding object-centric information individually.

\begin{figure}
  \centering
  \vspace{-0.5em}
  \includegraphics[width=0.9\linewidth]{content/figures/test_probe_complete.png}
  \caption{We visualize all bounding box predictions for each token in a frozen ResNet + Transformer encoder using probing.  We highlight the true positive bounding box predictions in green.}
  \vspace{-1em}
  \label{fig:probes_annotated}
\end{figure}
